Adaptive Scheduling of Data Paths using Uppaal Tiga

We apply Uppaal Tiga to automatically compute adaptive scheduling strategies for an industrial case study dealing with a state-of-the-art image processing pipeline of a printer. As far as we know, this is the first application of timed automata technology to an industrial scheduling problem with uncertainty in job arrivals.

==> eptcsdata.tex <==
\providecommand{\event}{S. Andova et.al. (Eds.): Workshop on Quantitative Formal Methods:\\ Theory and Applications (QFM'09) }
\providecommand{\volume}{13}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{1}
\providecommand{\eid}{1}
\pdfoutput=1

